3D Multi-Object Tracking Using Graph Neural Networks with Cross-Edge Modality Attention

Online 3D multi-object tracking (MOT) has witnessed significant research interest in recent years, largely driven by demand from the autonomous systems community. However, 3D offline MOT is relatively less explored. Labeling 3D trajectory scene data at a large scale while not relying on high-cost human experts is still an open research question. In this work, we propose Batch3DMOT which follows the tracking-by-detection paradigm and represents real-world scenes as directed, acyclic, and category-disjoint tracking graphs that are attributed using various modalities such as camera, LiDAR, and radar. We present a multi-modal graph neural network that uses a cross-edge attention mechanism mitigating modality intermittence, which translates into sparsity in the graph domain. Additionally, we present attention-weighted convolutions over frame-wise k-NN neighborhoods as suitable means to allow information exchange across disconnected graph components. We evaluate our approach using various sensor modalities and model configurations on the challenging nuScenes and KITTI datasets. Extensive experiments demonstrate that our proposed approach yields an overall improvement of 3.3% in the AMOTA score on nuScenes thereby setting the new state-of-the-art for 3D tracking and further enhancing false positive filtering.

==> sections/active_edges.tex <==
\begin{figure}[!htbp]
\captionsetup[subfigure]{justification=centering}
  \begin{subfigure}[t]{.45\textwidth}
  \begin{center}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.6cm,
            thick,
            gray/.style={fill=gray},
            yellow/.style={fill=yellow},
            blue/.style={fill=blue, text=white},
            red/.style={fill=red},
            green/.style={fill=green}]

\tikzstyle{every node}=[draw,shape=circle];
% first column
\node[draw, shape=circle,scale=0.02cm, label=above:{$t_{k,0}$}, gray] (yellow1) {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, green](green1) [below of=yellow1] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray](blue1) [below of=green1] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray](red1) [below of=blue1] {\,\,\,} ;

% second column
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,1}$}, gray] (yellow2) [right of=yellow1] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (green2) [below of=yellow2] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red2) [below of=green2] {\,\,\,} ;
%\node[shape=circle,scale=0.02cm, main node] (n8) [below of=red2] {8} ;

% third column
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,2}$}, gray] (yellow3) [right of=yellow2] {\,\,\,} ;
%\node[draw,shape=circle,scale=0.02cm, main node] (n10) [below of=n9] {10} ;
\node[draw,shape=circle,scale=0.02cm, green] (green3) [right of=red2] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red3) [below of=green3] {\,\,\,} ;

% fourth column
%\node[draw,shape=circle,scale=0.02cm, main node] (n13) [right of=n9] {13} ;
\node[draw=white, text=white,shape=circle,scale=0.02cm, label=above:{$t_{k,3}$}] (label4) [right of=yellow3] {\,\,\,};
\node[draw,shape=circle,scale=0.02cm, green] (green4) [right of=green3] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray] (blue4) [above of=green4] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red4) [below of=green4] {\,\,\,} ;

% fifth column
\node[draw,shape=circle,scale=0.02cm, green] (green5) [right of=blue4] {D} ;
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,4}$}, gray] (yellow5) [above of=green5] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (blue5) [below of=green5] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (gray5) [below of=blue5] {\,\,\,} ;


%green traj
\draw[->] (green4) to (green5);
\draw[->, bend left=5] (green3) to (green5);
\draw[->, bend left] (green1) to (green5);
\draw[->] (green3) to (green4);
\draw[->] (green1) to (green4);
\draw[->] (green1) to (green3);

\draw[->,dashed] (green4) to (green5);

%other_edges
\begin{scope}[transparency group, opacity=0.3] 
\draw[->, dashed] (red2) to (green3);
\draw[->, dashed] (red1) to (green3);

\draw[->, dashed] (yellow1) to (green2);

\draw[->, dashed] (green2) to (yellow3);
\draw[->, dashed] (green2) to (blue4);
\draw[->, dashed, bend left=15] (green2) to (green4);

\draw[->, dashed, bend left=15] (green2) to (yellow5);
\draw[->, dashed] (green3) to (red4);

\draw[->, dashed, bend left] (yellow3) to (green5);
\draw[->, dashed, bend left=10] (green4) to (yellow5);
\draw[->, dashed] (red4) to (green5);
\draw[->, dashed] (green4) to (gray5);

\draw[->, dashed, bend left=20] (yellow2) to (green4);
\draw[->, dashed] (green4) to (blue5);
\draw[->, dashed] (blue4) to (green5);
\end{scope}
\end{tikzpicture}
\end{center}
    \caption{Labeling all edges as active that exclusively connect the same object instance while satisfying DAG-constraints.}
    \label{fig:all_edges_instance}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.45\textwidth}
  \centering
    
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.8cm,
            thick,
            gray/.style={fill=gray},
            yellow/.style={fill=yellow},
            blue/.style={fill=blue, text=white},
            red/.style={fill=red},
            green/.style={fill=green}]

\tikzstyle{every node}=[draw,shape=circle];
% first column
\node[draw, shape=circle,scale=0.02cm, label=above:{$t_{k,0}$}, gray] (yellow1) {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, green](green1) [below of=yellow1] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray](blue1) [below of=green1] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray](red1) [below of=blue1] {\,\,\,} ;

% second column
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,1}$}, gray] (yellow2) [right of=yellow1] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (green2) [below of=yellow2] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red2) [below of=green2] {\,\,\,} ;
%\node[shape=circle,scale=0.02cm, main node] (n8) [below of=red2] {8} ;

% third column
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,2}$}, gray] (yellow3) [right of=yellow2] {\,\,\,} ;
%\node[draw,shape=circle,scale=0.02cm, main node] (n10) [below of=n9] {10} ;
\node[draw,shape=circle,scale=0.02cm, green] (green3) [right of=red2] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red3) [below of=green3] {\,\,\,} ;

% fourth column
%\node[draw,shape=circle,scale=0.02cm, main node] (n13) [right of=n9] {13} ;
\node[draw=white, text=white,shape=circle,scale=0.02cm, label=above:{$t_{k,3}$}] (label4) [right of=yellow3] {\,\,\,};
\node[draw,shape=circle,scale=0.02cm, green] (green4) [right of=green3] {D} ;
\node[draw,shape=circle,scale=0.02cm, gray] (blue4) [above of=green4] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (red4) [below of=green4] {\,\,\,} ;

% fifth column
\node[draw,shape=circle,scale=0.02cm, green] (green5) [right of=blue4] {D} ;
\node[draw,shape=circle,scale=0.02cm, label=above:{$t_{k,4}$}, gray] (yellow5) [above of=green5] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (blue5) [below of=green5] {\,\,\,} ;
\node[draw,shape=circle,scale=0.02cm, gray] (gray5) [below of=blue5] {\,\,\,} ;


%green traj
\draw[->] (green4) to (green5);
\draw[->] (green3) to (green4);
\draw[->] (green1) to (green3);




%other_edges
\begin{scope}[transparency group, opacity=0.3] 
\draw[->, dashed, bend left=5] (green3) to (green5);
\draw[->, dashed, bend left] (green1) to (green5);
\draw[->, dashed] (green1) to (green4);
\draw[->, dashed] (red2) to (green3);
\draw[->, dashed] (red1) to (green3);

\draw[->, dashed] (yellow1) to (green2);

\draw[->, dashed] (green2) to (yellow3);
\draw[->, dashed] (green2) to (blue4);
\draw[->, dashed, bend left=15] (green2) to (green4);

\draw[->, dashed, bend left=15] (green2) to (yellow5);
\draw[->, dashed] (green3) to (red4);

\draw[->, dashed, bend left] (yellow3) to (green5);
\draw[->, dashed, bend left=10] (green4) to (yellow5);
\draw[->, dashed] (red4) to (green5);
\draw[->, dashed] (green4) to (gray5);

\draw[->, dashed, bend left=20] (yellow2) to (green4);
\draw[->, dashed] (green4) to (blue5);
\draw[->, dashed] (blue4) to (green5);
\end{scope}
\end{tikzpicture}
    \caption{Connecting only time-nearest detections via active edges in order to emphasize model learning w.r.t.\ false negatives.}
    \label{fig:only_adjacent_edges}
  \end{subfigure}
  \caption[Two edge construction paradigms]{Edge construction. There are two different ways to label active graph edges. Either connecting all detections (a) or only nearest detections (b) per object instance under time-positive directedness.}
  \label{fig:active_edges}
\end{figure}
